The fifth-order post-Newtonian Hamiltonian dynamics of two-body systems from an effective field theory approach

Within an effective field theory method to general relativity, we calculate the fifth-order post--Newtonian (5 PN) Hamiltonian dynamics also for the tail terms, extending earlier work on the potential contributions, working in harmonic coordinates. Here we calculate independently all (local) 5 PN contributions to the tail terms using the in--in formalism, on which we give a detailed account. The five expansion terms of the Hamiltonian in the effective one body (EOB) approach, $q_{82}, q_{63}, q_{44}, \bar{d_5}$ and $a_6$, can all be determined from the local contributions to periastron advance $K^{\rm loc,h}(\hat{E},j)$, without further assumptions on the structure of the symmetric mass ratio, $\nu$, of the expansion coefficients of the scattering angle $\chi_k$. The $O(\nu^2)$ contributions to the 5 PN EOB parameters have been unknown in part before. We perform comparisons of our analytic results with the literature and also present numerical results on some observables.

==> FR1.tex <==
%\allowdisplaybreaks
\begin{align}
%
  \phi:\raisebox{-5.1mm}{\includegraphics{phiprop}} ={}& - \frac{i}{2c_d} D(p)\,,\displaybreak[0]\\
%
  A:\raisebox{-5.1mm}{\includegraphics{Aprop}} ={}& \frac{i\delta_{ij}}{2} D(p)\,,\displaybreak[0]\\
%
  \sigma:\raisebox{-5.1mm}{\includegraphics{sigmaprop}} ={}&
-\frac{i}{2}D(p)[\delta_{i_1j_1}\delta_{i_2j_2} + \delta_{i_1j_2}\delta_{i_2j_1} +
(2-c_d)\delta_{i_1i_2}\delta_{j_1j_2}]\,,\displaybreak[0]\\ %
  \centeredgraphics{vphibinary} ={}& -\frac{i}{\Lambda} \biggl(
E
{-} \frac{1}{2} Q_{ij}p_i p_j
{-} \frac{i}{6} O_{ijk} p_i p_j p_k
\biggr)\,,\\
%
  \centeredgraphics{vAbinary} ={}& \frac{i}{\Lambda} \biggl(
- \frac{i}{2} L_{j}\varepsilon_{ijk} p_k
{-} \frac{1}{2} Q_{ij} p_0 p_j
+ \frac{1}{3} J_{jk} \varepsilon_{ijl} p_k p_l
{-} \frac{i}{6} O_{ijk} p_j p_k p_0
\biggr)\,,\\
%
\label{eq:FR1}
  \centeredgraphics{vsigmabinary} ={}& \frac{i}{\Lambda} \biggl(
- \frac{1}{4} Q_{ij} p_0^2
+ \frac{1}{6}(J_{ik}\varepsilon_{jkl} + J_{jk}\varepsilon_{ikl}) p_l p_0
{-} \frac{i}{12} O_{ijk} p_k p_0^2
\biggr)\,,\\
%
\label{eq:FR2}
  \centeredgraphics{vsigmasigmabinary} ={}&
\begin{aligned}
\tfrac{i}{16\Lambda^2} p_{1 0} p_{2 0} (&
 \delta_{i_1 i_2} Q_{j_1 j_2}
+ \delta_{i_1 j_2} Q_{i_2 j_1}\\
&+ \delta_{i_2 j_1} Q_{i_1 j_2}
+ \delta_{j_1 j_2} Q_{i_1 i_2}
+ \dots
)\,,
\end{aligned}\\
%
\label{e114}
  \centeredgraphics{vphiphiphi} ={}& \frac{2i c_d^2}{\Lambda} (p_{10} p_{20} + p_{10} p_{30} + p_{20} p_{30})\,,\\
%
\label{e115}
  \centeredgraphics{vphiphiA} ={}& -\frac{2i c_d}{\Lambda} (p_{10} p_{2i_3} + p_{1i_3} p_{20})\,,\\
%
\label{e116}
  \centeredgraphics{vphiphisigma} ={}& \frac{i c_d}{\Lambda} (-p_{1_3i} p_{2j_3} - p_{1j_3} p_{2i_3} + \delta_{i_3j_3} p_1\cdot p_2)\,,\\
%
\label{e117}
  \centeredgraphics{vphiAA} ={}& \frac{2i c_d}{\Lambda}(-p_{2i_2} p_{3i_3} + p_{2i_3} p_{3i_2} - 2 \delta_{i_2
i_3} p_{2i} p_{3i}) \,,\\
%
\label{e118}
  \centeredgraphics{vphiAsigma} ={}&
\begin{aligned}
\tfrac{i c_d}{\Lambda}(&
- \delta_{i_3 i_2} p_{1 0} p_{2 i_3}
+ \delta_{i_3 i_2} p_{1 j_3} p_{2 0}
+ \delta_{i_3 j_3} p_{1 0} p_{2 i_2}\\
&- \delta_{i_3 j_3} p_{1 i_2} p_{2 0}
- \delta_{i_2 j_3} p_{1 0} p_{2 i_3}
+ \delta_{i_2 j_3} p_{1 i_3} p_{2 0}
)\,,
\end{aligned}
\\
%
\label{e119}
    \centeredgraphics{vphisigmasigma} ={}& \frac{i c_d}{2\Lambda} p_{2 0} p_{3 0} (
  \delta_{i_2 i_3} \delta_{j_2 j_3}
- \delta_{i_2 j_2} \delta_{i_3 j_3}
+ \delta_{i_2 j_3} \delta_{i_3 j_2}
)\,,\\
%
\label{e120}
\centeredgraphics{vAAA} ={}&
\begin{aligned}
\tfrac{2i}{\Lambda} (
&- \delta_{i_1 i_2} p_{1 0} p_{2 i_3}
- \delta_{i_1 i_2} p_{1 0} p_{3 i_3}
+ \delta_{i_1 i_2} p_{1 i_3} p_{2 0}
+ \delta_{i_1 i_2} p_{1 i_3} p_{3 0}\\
&+ \delta_{i_1 i_2} p_{2 0} p_{3 i_3}
+ \delta_{i_1 i_2} p_{2 i_3} p_{3 0}
+ \delta_{i_1 i_3} p_{1 0} p_{2 i_2}
+ \delta_{i_1 i_3} p_{1 0} p_{3 i_2}\\
&- \delta_{i_1 i_3} p_{1 i_2} p_{2 0}
+ \delta_{i_1 i_3} p_{1 i_2} p_{3 0}
- \delta_{i_1 i_3} p_{2 0} p_{3 i_2}
+ \delta_{i_1 i_3} p_{2 i_2} p_{3 0}\\
&+ \delta_{i_2 i_3} p_{1 0} p_{2 i_1}
+ \delta_{i_2 i_3} p_{1 0} p_{3 i_1}
+ \delta_{i_2 i_3} p_{1 i_1} p_{2 0}
- \delta_{i_2 i_3} p_{1 i_1} p_{3 0}\\
&+ \delta_{i_2 i_3} p_{2 0} p_{3 i_1}
- \delta_{i_2 i_3} p_{2 i_1} p_{3 0}
)\,,
\end{aligned}
\\
%
\label{e121}
  \centeredgraphics{vAAsigma} ={}&
\begin{aligned}
\tfrac{i}{\Lambda} (
&p_1\cdot p_2 (
- \delta_{i_1 i_2} \delta_{i_3 j_3}
+ \delta_{i_1 i_3} \delta_{i_2 j_3}
+ \delta_{i_2 i_3} \delta_{i_1 j_3}
)\\
&+ \delta_{i_1 i_2} (p_{1 i_3} p_{2 j_3} + p_{1 j_3} p_{2 i_3})
+ \delta_{i_1 i_3} (p_{1 i_2} p_{2 j_3} - p_{1 j_3} p_{2 i_2})\\
&- \delta_{i_2 i_3} (p_{1 i_1} p_{2 j_3} - p_{1 j_3} p_{2 i_1})
+ \delta_{i_1 j_3} (p_{1 i_2} p_{2 i_3} - p_{1 i_3} p_{2 i_2})\\
&- \delta_{i_2 j_3} (p_{1 i_1} p_{2 i_3} - p_{1 i_3} p_{2 i_1})
+ \delta_{i_3 j_3} (p_{1 i_1} p_{2 i_2} - p_{1 i_2} p_{2 i_1})
)\,,
\end{aligned}
\\
%
\label{e122}
\centeredgraphics{vAsigmasigma} ={}&
\frac{i}{8\Lambda}(V^{A\sigma\sigma}_{i_1,i_2j_2,i_3j_3}
+ V^{A\sigma\sigma}_{i_1,i_2j_2,j_3i_3}
+ V^{A\sigma\sigma}_{i_1,j_2i_2,i_3j_3}
+ V^{A\sigma\sigma}_{i_1,j_2i_2,j_3i_3})\\
V^{A\sigma\sigma}_{i_1,i_2j_2,i_3j_3}={}&\delta_{i_{2} i_{3}} \delta_{j_{2} j_{3}} [4 p_{20} p_{2i_{1}}+2 (p_{1i_{1}} p_{20}+p_{10} p_{2i_{1}})]+\delta_{i_{3} j_{3}} [-2 p_{20} (\delta_{i_{1} i_{2}} p_{1j_{2}}\notag\\
&      +\delta_{i_{2} j_{2}} p_{2i_{1}})-\delta_{i_{2} j_{2}} (p_{1i_{1}} p_{20}+p_{10} p_{2i_{1}})]+\delta_{i_{1} i_{2}} [2 \delta_{i_{3} j_{3}} p_{10} p_{2j_{2}}\notag\\
&   +\delta_{i_{3} j_{2}} (4 p_{1j_{3}} p_{20}-4 p_{10} p_{2j_{3}})]+\delta_{i_{1} i_{3}} [\delta_{i_{2} j_{3}} (-4 p_{1j_{2}} p_{20}\notag\\
&      +4 p_{10} p_{2j_{2}})+\delta_{i_{2} j_{2}} (2 p_{1j_{3}} p_{20}-2 p_{10} p_{2j_{3}})] \\
%
\label{e124}
  \centeredgraphics{vsigmasigmasigma} ={}& \frac{i}{32\Lambda}(\tilde{V}^{\sigma\sigma\sigma}_{i_1j_1,i_2j_2,i_3j_3} +
       \tilde{V}^{\sigma\sigma\sigma}_{j_1i_1,i_2j_2,i_3j_3})\\
  \tilde{V}^{\sigma\sigma\sigma}_{i_1j_1,i_2j_2,i_3j_3} ={}&
       V^{\sigma\sigma\sigma}_{i_1j_1,i_2j_2,i_3j_3} +
       V^{\sigma\sigma\sigma}_{i_1j_1,j_2i_2,i_3j_3} +
       V^{\sigma\sigma\sigma}_{i_1j_1,i_2j_2,j_3i_3} +
  V^{\sigma\sigma\sigma}_{i_1j_1,j_2i_2,j_3i_3}
\displaybreak[0]\\
V^{\sigma\sigma\sigma}_{i_1j_1,i_2j_2,i_3j_3}
={}&({p}_1^2+{p}_1\cdot{p}_2+{p}_2^2)\*\Bigl(-\delta_{i_2j_2}\*\bigl(2\*\delta_{i_1i_3}\*
\delta_{j_1j_3}-\delta_{i_1j_1}\*\delta_{i_3j_3}\bigr)
\notag\\
&\quad+2\*\bigl[\delta_{i_1i_2}\*\bigl(4\*\delta_{j_1i_3}\*\delta_{j_2j_3}-\delta_{j_1j_2}\*\delta_{i_3j_3}\bigr)
-\delta_{i_1j_1}\*\delta_{i_2i_3}\*\delta_{j_2j_3}\bigr] \Bigr)
\notag\\
&+2\*\Bigl\{4\*\bigl(p_{1 j_3}\*p_{2 j_1}-p_{1 j_1}\*p_{2 j_3}\bigr)\*\delta_{i_1i_2}\*\delta_{j_2i_3}
\notag\\
&\quad+2\*\bigl[\bigl(p_{1 i_1}+p_{2 i_1}\bigr)\*p_{2 j_1}\*\delta_{i_2i_3}\*\delta_{j_2j_3}-p_{1 i_3}\*p_{2 j_3}\*
\delta_{i_1i_2}\*\delta_{j_1j_2}\bigr]
\notag\\
&\quad+\delta_{i_2j_2}\*\bigl[p_{1 i_3}\*p_{2 j_3}\*\delta_{i_1j_1}+2\*\bigl(p_{1 j_3}\*p_{2 j_1}-p_{1 j_1}\*
p_{2 j_3}\bigr)\*\delta_{i_1i_3}\notag\\
&\quad-\bigl(p_{1 i_1}+p_{2 i_1}\bigr)\*p_{2 j_1}\*\delta_{i_3j_3}\bigr]
\notag\\
&\quad+p_{2 j_2}\*\Bigl(4\*p_{1 j_1}\*\delta_{i_1i_3}\*\delta_{i_2j_3}+p_{1 i_2}\*\bigl(2\*\delta_{i_1i_3}\*
\delta_{j_1j_3}-\delta_{i_1j_1}\*\delta_{i_3j_3}\bigr)
\notag\\
&\qquad+2\*\bigl[\delta_{i_1i_2}\*\bigl(p_{1 j_1}\*\delta_{i_3j_3}-2\*p_{1 j_3}\*\delta_{j_1i_3}\bigr)-p_{1 j_3}\*
\delta_{i_1j_1}\*\delta_{i_2i_3}\bigr] \Bigr)
\notag\\
&\quad+p_{1 j_2}\*\Bigl(p_{1 i_2}\*\bigl(2\*\delta_{i_1i_3}\*\delta_{j_1j_3}-\delta_{i_1j_1}\*\delta_{i_3j_3}\bigr)
-4\*p_{2 j_1}\*\delta_{i_1i_3}\*\delta_{i_2j_3}
\notag\\
&\qquad+2\*\bigl[p_{2 j_3}\*\delta_{i_1j_1}\*\delta_{i_2i_3}+\delta_{i_1i_2}\*\bigl(2\*p_{2 j_3}\*\delta_{j_1i_3}
-p_{2 j_1}\*\delta_{i_3j_3}\bigr)\bigr]
\Bigr)\Bigr\},
\end{align}

